Mirage: Towards Deployable DDoS Defense for Web Applications

Distributed Denial of Service (DDoS) attacks form a serious threat to the security of Internet services. However, despite over a decade of research, and the existence of several proposals to address this problem, there has been little progress to date on actual adoption. We present Mirage, a protocol that achieves comparable performance to other DDoS mitigation schemes while providing benefits when deployed only in the server's local network and its upstream ISP, where local business objectives may incentivize deployment. Mirage does not require source end hosts to install any software to access Mirage protected websites. Unlike previous proposals, Mirage only requires functionality from routers that is already deployed in today's routers, though this functionality may need to be scaled depending on the point of deployment. Our approach is that end hosts can thwart the attackers by employing the principle of a moving target: end hosts in our architecture periodically change IP addresses to keep the attackers guessing. Knowledge of an active IP address of the destination end host can act as an implicit authorization to send data. We evaluate Mirage using theoretical analysis, simulations and a prototype implementation on PlanetLab. We find that our design provides a first step towards a deployable, yet effective DDoS defense.

==> evaluation_old.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we evaluate the effectiveness and the efficiency of
Mirage. In particular, we quantify the attack resilience of Mirage
using a prototype implementation and an ns-2 simulation, and we
perform Internet bandwidth measurements to determine the extent to
which Mirage must be deployed in order to provide protection against
various levels of DoS. %, and compare the costs of various DoS
%defense mechanisms.




%\paragraphb{Experimental Validation:} We now describe implementation results that validate our
%architecture. We implemented Mirage on the Emulab framework~\cite{emulab}.
%We use the topology of the Abilene network~\cite{abeline} as our network topology. We set the latency
%between routers using $2/3$'rds the speed of light over their geographic distance. Since we are interested
%in studying the effect of congestion due to denial of service attacks, we scale down the link bandwidth
%between routers to $10$Mb, and the last hop bandwidth to $1$Mb.


%We first examine the effect of the attack traffic
%rate on the benign traffic. To this end, we set up ten benign TCP traffic
%flows and one UDP attack traffic flows that share a single bottleneck link
%to the victim. We measured the throughput of the benign and the attack traffic.
%Figure~\ref{fig:results}b shows our measurements when we vary the attack
%traffic rate from $0.1$Mbps to $1$Mbps (bottleneck bandwidth). We can see that
%the throughput of the benign traffic is very close to its fair share regardless
%of the attack traffic rate.
%%fair queueing in Mirage guarantees the throughput of benign traffic for various attack
%%traffic rates, regardless of the attack traffic rate.

%Next, we provide a comparison between Mirage and a filter-based approach.  The
%performance of a filter-based scheme depends on its ability to classify attack
%traffic.  However, it is difficult to accurately classify attack traffic under
%sophisticated attacks.  Thus, we vary the fraction of attack traffic that can
%be classified (detection ratio), and measure the throughput of benign traffic
%and attack traffic, assuming {\em perfect filtering of classified traffic}. For
%this experiment, we use $10$ UDP-based attack flows.  Figure~\ref{fig:results}c
%shows that when the detection rate is low, a pure filter-based approach results
%on low throughput for benign flows. In contrast, Mirage guarantees a  fair
%share for the benign traffic. On the other hand, the performance of both schemes
%is comparable when the detection rate is high.

%\begin{figure*}[t]
%\centering
%\mbox{ \hspace{-0.2in} \hspace{-0.12in}
%\begin{tabular}{c}
%%\psfig{figure=figs/tbd.eps,height=1.5in}\vspace{-0.00in}\\
%\includegraphics[width=0.7\columnwidth,clip]{figs/fair_queueing_evaluation} \\
%{(a)}
%\end{tabular}
%\hspace{-0.12in}
%\begin{tabular}{c}
%%\psfig{figure=figs/tbd.eps,height=1.5in}\vspace{-0.00in}\\
%\includegraphics[width=0.7\columnwidth,clip]{figs/tput_filtered_attacker} \\
%{(b)}
%\end{tabular}
%} \caption{{\em } (a) Fair queueing guarantees normal users'
%throughput even with high-rate attackers. (b) While Mirage
%guarantees fair share for benign flows regardless of the detection
%ratio, a filter-based scheme is not sufficient when the detection
%rate is low. } \label{fig:results}
%\end{figure*}


\subsection{Prototype Implementation} \label{sec:prototype_impl}
%\begin{figure*}[!t]
%\centerline{ \subfigure[The architecture of our prototype
%implementation:
%]{\includegraphics[width=0.45\textwidth]{figs/prototype_impl}\label{fig:prototype_impl}}
%%\hspace{6pt}
%\subfigure[Experimental setup based on our prototype implementation:
%we interconnect users (legitimate users and attackers), router and
%DNS server via UDP-encapsulated tunnel.
%]{\includegraphics[width=0.45\textwidth]{figs/planetlab_exp}\label{fig:planetlab_exp}}
%}%\vspace{-9pt}
%\caption{ }%\vspace{-10pt}
%\label{fig:exp_impl_architecture}
%\end{figure*}

%To evaluate performance and to grapple with operational and deployment issues, we implemented a prototype of our
%design (~\ref{fig:prototype_impl}).

%\matt{
To evaluate its performance and to grapple with deployment issues, we built
a prototype implementation of Mirage. %}
Figure~\ref{fig:prototype_impl} shows the basic architecture of our
prototype system. We did not attempt to optimize the prototype
system; rather, our goal is to verify the design and evaluate its
deployability. To evaluate our prototype, we constructed a {\em
Mirage-enabled web service}, which we call the \emph{victim server},
and configured a set of clients to access that web service.

\paragraphb{Client side:}
We implemented the JavaScript program described in
Section~\ref{sec:javascript_extension} to enable
the client to ``hop'' addresses without requiring changes to the
browser or operating system code running at the client.
%\mattc{ah, so you don't require changes to the browser or operating system code at the client. this is the first time in the paper where I figured that out, if this is actually true you should mention this earlier, once section 4-5, possibly once again in sections 1-3.}
This JavaScript program at the puzzle server
as shown in Figure~\ref{fig:prototype_impl}.
When the DNS directs a client to the puzzle server,
the client fetches and solves the puzzle by running the JavaScript code
provided by the puzzle server.
These operations are transparent to the user;
the user simply directs its web browser
to the domain name of the victim server.

\paragraphb{Server side:}
The server-side components,
comprised of the victim server, router, DNS server, and puzzle server,
provide \emph{transparent} protection for a victim server.
By transparent, we mean that the user of a client machine
need not install any additional software.
%\mattc{oh, it's the first time you're mentiong this too, that's neat. If this is actually true, seems like it should be mentioned earlier}

\begin{figure}
    \centering
    \includegraphics[width=0.42\textwidth]{figs/prototype_impl}
    \caption{
    The architecture of our prototype implementation. %all servers (including router) are implemented in Linux.
    To initiate a connection to a destination,
    the client first performs a domain name resolution
    through a DNS server.
    The DNS server implements failover to Mirage
     by regularly checking the status of the victim server.
    When the destination becomes unavailable,
     the DNS server provides the IP address of a puzzle server instead.
    The client fetches a puzzle from a puzzle server
     to get a hopping address, %\mattc{hopping address or Mirage address?}
    and redirects its frame to the hopping address.
    The target server, router, DNS server, and puzzle server
     share a common key and have loosely synchronized clocks
     in order to generate hopping addresses.
    Tight time synchronization is not required, as explained
     in Section~\ref{sec:destination}.
}
    \label{fig:prototype_impl}
\end{figure}
%This transparent protection feature is enabled by the
%DNS server checking the status of the target server and redirection
%in a client web browser.

%In our implementation, we assumed that all server side components
%share a common key to generate hopping address. AES

We used BIND~\cite{tool:bind} to implement the DNS server. We
defined our own zone (miragev6.org) and created a probing tool that
regularly send pings to the victim server to detect when the victim
server is under attack. Initially, www.miragev6.org resolves
directly to the victim's IP address. Once the probing tool fails to
receive a certain number of echo responses, it changes the DNS
record so that www.miragev6.org resolves to the puzzle server's IP
address (which, in our prototype, is the DNS server). We set the TTL
for the DNS record to a small value so that an entry cached before
the victim was under attack will be quickly corrected once the
victim is under attack.

When the victim is under DoS attack and
the client tries to access www.miragev6.org,
the client receives the IP address of the puzzle server.
The client connects to the puzzle server and fetches a piece of JavaScript
which includes a puzzle.
Our implementation uses the scheme described in Section~\ref{sec:puzzle},
using AES as the encryption algorithm.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.48\textwidth]{figs/planetlab_exp}
    \caption{Experimental setup based on our prototype implementation.
    To evaluate our system in a real Internet environment,
    we use PlanetLab nodes.
    Because PlanetLab nodes are protected by firewalls and lack IPv6 support,
    we interconnect users (both legitimate users and attackers), routers,
    and the DNS server using a UDP-encapsulated tunnel implemented in Click.}
    \label{fig:planetlab_exp}
\end{figure}

%\noindent \textbf{Experimental setup.}
\paragraphb{Experimental setup:}
%\matt{
To investigate Mirage's operation in the wide-area, we conducted
experiments in the Internet using the PlanetLab testbed.
Figure~\ref{fig:planetlab_exp} shows how we set up the network. We
selected random (lightly CPU-loaded) nodes to run our experiments.
We selected one PlanetLab node to act as the client, and one
PlanetLab node to run the server, router, puzzler server, and DNS
software. Since PlanetLab hosts do not directly provide IPv6
compatibility, for our IPv6 experiments we used an IPv4 encapsulated
tunnel. We found that standard tunnel (e.g. GRE) packets are blocked
by firewalls of some PlanetLab networks, so we used UDP tunnels for
our experiments. We implemented this tunnel with the
TUN~\cite{tool:tuntap} virtual interface and
Click~\cite{tool:click}. In an IPv6-enabled machine, outgoing IPv6
packets are delivered to TUN device which lets Click capture the
packets. Click then encapsulates the packets with UDP tunnel.
Because PlanetLab nodes lack kernel support for IPv6, we assigned
IPv4 addresses to the TUN device and used Click to translate between
IPv4 and IPv6 addresses.

%d% The basic goal in our experiments is to evaluate Mirage in a real-world environment.
%d% The Internet is the natural candidate for us. Unfortunately, since we could not utilize public IPv6 network, we used IPv4-encapsulated tunnel. Figure~\ref{fig:planetlab_exp} shows how we set up the network. To reflect on actual traffic condition in the Internet, we use
%d% PlanetLab~\cite{tool:planetlab} nodes and our lab machines. Since standard tunnel (e.g. GRE) packets are blocked by firewall of our networks,
%d% we use UDP tunnel. Hence, our IPv6 packets are encapsulated by UDP header and IPv4 header.
%d% We implemented this tunnel by a virtual interface called TUN~\cite{tool:tuntap} and Click~\cite{tool:click}.
%d% In IPv6-enabled machine, outgoing IPv6 packets are delivered to TUN device which let Click capture the packets. Click encapsulates
%d% the packets with UDP tunnel. PlanetLab node does not support IPv6 stack in its kernel. Hence, we assign IPv4 address in TUN device in
%d% PlanetLab nodes and let Click converts IPv4 address to IPv6 address vice versa.

\subsection{Effectiveness}

In this section, we evaluate how well Mirage can defend against
possible attacks. We do not argue that we consider all possible
attacks; rather, our intention is to quantify Mirage's attack
resilience. %\mattc{
Furthermore, because we only implement some of
the Mirage functionality described in this paper, we explicitly do
not consider attacks that are solved by unimplemented parts of
Mirage. %}
We consider two attacks: one that exhausts network
bandwidth and one that exhausts hopping IP addresses.

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.42\textwidth]{figs/fair_queueing_evaluation}
    \caption{Mirage guarantees normal users' throughput even with high-rate attackers.}
    \label{fig:fair_queueing_evaluation}
\end{figure}

\paragraphb{Bandwidth exhaustion attack:}
By increasing its sending rate,
or by increasing the number of flows it sends,
an attacker can increase its traffic rate
to overwhelm normal users' traffic.
We examined the effect of the attack traffic rate on benign traffic
by setting up
%To this end, we set up
ten benign TCP traffic flows and one UDP attack traffic flow
that share a single bottleneck link to the victim.
We measured the throughput of the benign and the attack traffic,
and compared their throughputs with and without Mirage.
Figure~\ref{fig:fair_queueing_evaluation} shows the results
when we vary the attack traffic rate between 0.5 to 1.3 times
the bandwidth of the bottleneck link.
Without Mirage, as the attack traffic rate increases,
the normal user's traffic rate decreases;
however, in Mirage,
fair queueing drops the attackers' excess packets
rather than the normal user's traffic.

\begin{figure*}[!t]
\centerline{ \subfigure[Implementation study with a small number of
attacker processes (the number of attacker machines = 3)
]{\includegraphics[width=0.32\textwidth]{figs/puzzle_evaluation_ratio}\label{fig:puzzle_evaluation_small_scale}}
\hspace{4pt} \subfigure[Simulation study with a large number of
attacker processes (the number of attacker machines = 3)
]{\includegraphics[width=0.32\textwidth]{figs/puzzle_many_attacker_num_machine_3}\label{fig:puzzle_evaluation_machine_3}}
\hspace{4pt} \subfigure[Simulation study with a large number of
attacker processes (the number of attacker machines = 30)
]{\includegraphics[width=0.32\textwidth]{figs/puzzle_many_attacker_num_machine_30}\label{fig:puzzle_evaluation_machine_30}}
}%\vspace{-9pt}
\caption{The puzzle system in Mirage limits the ability of an attacker to obtain too many hopping IP addresses.}%\vspace{-10pt}
\label{fig:puzzle_evaluation}
\end{figure*}

\paragraphb{Hopping IP address exhaustion attack:}
Since Mirage uses fair queueing per hopping IP address, an attacker
can request a large number of hopping IP addresses to prevent normal
users from getting hopping IP addresses, thus preventing normal
users from transmitting to the victim. In order to evaluate Mirage's
performance under a large number of attackers, we use the ns-2
network simulator~\cite{simulator:ns}. To parametrize the
simulation, we developed a computational model and used Internet
experiments using a small number of attacker processes to estimate
the parameters for our model.

Our Internet experiments used three machines to behave as an
attacker and one machine to behave as the normal user. We used
Firefox to access the Mirage-enabled web service. Both normal users
and attackers solve puzzles as quickly as possible in order to
obtain hopping addresses; however, in normal user machines, a single
Firefox process generates IP addresses, whereas on attacker
machines, we vary the number of Firefox processes that are
generating IP addresses.
%The number of attacker flows in the result graph
%(Figure~\ref{fig:puzzle_evaluation_small_scale})
%corresponds to the number of Firefox processes.
%\mattc{I think we can just repalce ``flows'' with
%``Attack processes / machine'': need to do this in the figure too}
We used Selenium~\cite{tool:selenium} to
remotely control the Firefox processes.
In our prototype implementation,
the puzzle server uses hopping IP addresses released from a leaky bucket
and assigns it to the puzzle solution with the highest difficulty.
%the chosen flow will get a hopping IP address.
A process that is not chosen will increase its puzzle difficulty and
try again. Without Mirage, the puzzle server grants all requests for
IP addresses. We measured the number of hopping IP addresses
obtained by the attacker machines and the normal user machine.
Figure~\ref{fig:puzzle_evaluation_small_scale} shows the ratio of
the number of hopping IP addresses per attacker machine to the
number of hopping IP addresses of normal user machine. Without
Mirage, as the number of attacker processes increases, the attacker
machine can get a larger number of hopping IP addresses, which
corresponds to a large number of victim machine accesses. The growth
rate becomes smaller as the number of processes increases because
the additional processes will saturate the machine's computational
power. With Mirage, this computational limit is reached much more
quickly, because a node's ability to get IP addresses is
computationally limited.

We used this experimental data to establish a model in ns-2. We used
a dumbbell topology with RTT equal to that from our experimental
study. When a node solves a puzzle solution, it takes an amount of
time to generate a solution given by
\begin{displaymath}
\frac{B+N \times E }{C}%Base\_load+Num\_try \times Solution\_calculation}{Computation\_power}
\end{displaymath}
where $B$ is the cost (in cycles)
of running Firefox without puzzle calculations,
$N$ represents the number of encryption attempts
needed to solve a puzzle, which we model as a normal distribution,
$E$ is the number of cycles taken by each encryption attempt,
and $C$ is the speed of the CPU.
%\mattc{Confused about your description of N?}
%how many a Firefox process uses encryption algorithm to get a puzzle solution.
%\mattc{can't someone complain that firefox is a heavyweight thiing
%as shown by the no-mirage results, and that the attacker should do better
%using something like wget+custom code vs firefox?}
%We used uniform distribution to model $N$. %\mattc{you never
%say what Num try actually is, much less the other variables}.
%$E$ represents how long it takes to perform a single encryption algorithm.
%$C$ represents the speed of CPU.
Without Mirage, a node takes time $B/C$ to
resolve the victim's IP address.
We varied the values of $B$, $N$, and $E$ to find parameters
that best matched our experimental study;
that is, ones that minimized the variance
between experimental and simulation results.
%We exhaustively \mattc{how?} searched for
%a good set of parameters to match our experimental situation by
%varying the values of the three parameters. We chose the parameters
%to maximally reduce the variance of the difference of experimental
%data and simulation data.
Figure~\ref{fig:puzzle_evaluation_small_scale} shows how well the
two sets of data match.

With these simulation parameters, we performed simulation studies to
show how the number of attacker processes affects the number of
hopping IP addresses that the attacker machine obtained.
Figure~\ref{fig:puzzle_evaluation_machine_3} and
Figure~\ref{fig:puzzle_evaluation_machine_30} show the results when
the number of attacking machines is 3 and 30, respectively. We vary
the number of attacker processes from 3 to 30000. In all cases, we
can see that the attacker in Mirage cannot obtain as many hopping IP
addresses as the case without Mirage.





\input{bottleneck-computations}

%\input{comparison_overhead}

